Web News Timeline Generation with Extended Task Prompting

The creation of news timeline is essential for a comprehensive and contextual understanding of events as they unfold over time. This approach aids in discerning patterns and trends that might be obscured when news is viewed in isolation. By organizing news in a chronological sequence, it becomes easier to track the development of stories, understand the interrelation of events, and grasp the broader implications of news items. This is particularly helpful in sectors like finance and insurance, where timely understanding of the event development-ranging from extreme weather to political upheavals and health crises-is indispensable for effective risk management. While traditional natural language processing (NLP) techniques have had some success, they often fail to capture the news with nuanced relevance that are readily apparent to domain experts, hindering broader industry integration. The advance of Large Language Models (LLMs) offers a renewed opportunity to tackle this challenge. However, direct prompting LLMs for this task is often ineffective. Our study investigates the application of an extended task prompting technique to assess past news relevance. We demonstrate that enhancing conventional prompts with additional tasks boosts their effectiveness on various news dataset, rendering news timeline generation practical for professional use. This work has been deployed as a publicly accessible browser extension which is adopted within our network.

==> figures/f1_dataset_scores.tex <==
\caption{F1 scores for different dataset}
\begin{adjustbox}{width=1\linewidth}

\begin{tabular}{ |c|ccc|ccc|ccc|} 
    \hline
  & \multicolumn{3}{c|}{Vicuna-7b-v1.5} & \multicolumn{3}{c|}{GPT-3.5-turbo} & \multicolumn{3}{c|}{GPT-4-1106-preview} \\
    \hline
 & crisis & t17 & news & crisis & t17 & news & crisis & t17 & news \\
 \hline
 
 
 Direct &  0.516 & 0.594 & 0.583 & 0.738 & 0.671 & 0.728 & 0.865 & 0.841 & 0.817

 
 \\
 % Explain & 0.769 & 0.621 & 0.648 & 0.598 & 0.856 & 0.672 \\
 Summary &   \textbf{0.687} & \textbf{0.738} & \textbf{0.715} & \textbf{0.819} & \textbf{0.730} & \textbf{0.758} & \textbf{0.865} & \textbf{0.852} & \textbf{0.827}


 \\
 \hline
\end{tabular}
\end{adjustbox}

==> figures/f1_dataset_scores_one_column.tex <==
\begin{tabular}{ |c|ccc|} 
  %   \hline
  % & \multicolumn{3}{c|}{Vicuna-7b-v1.5} & \multicolumn{3}{c|}{GPT-3.5-turbo} & \multicolumn{3}{c|}{GPT-4-1106-preview} \\
    \hline
dataset & Crisis & TL17 & news\\
\hline
   & \multicolumn{3}{c|}{Vicuna-7b-v1.5}
 
 \\
 Basic &  0.516 & 0.594 & 0.583 \\
 Extended &   \textbf{0.687} & \textbf{0.738} & \textbf{0.715} 
 \\
 \hline & \multicolumn{3}{c|}{GPT-3.5-turbo} \\
 
 Basic  & 0.738 & 0.671 & 0.728 \\
  Extended &    \textbf{0.819} & \textbf{0.730} & \textbf{0.758}  \\

  
 \hline  & \multicolumn{3}{c|}{GPT-4-1106-preview}\\ 
 
 Basic &  0.865 & 0.841 & 0.817 \\
  Extended & \textbf{0.865} & \textbf{0.852} & \textbf{0.827} \\
  
 \hline
\end{tabular}


==> figures/prompt_evaluation.tex <==
\caption{\textsc{Storyline labelling performance for \basicprompt and \extendedprompt}}
 \extendedprompt &   \textbf{0.687} & \textbf{0.738} & \textbf{0.715} 
\begin{adjustbox}{width=1\linewidth}

\begin{tabular}{ |c|ccc|ccc|ccc|} 
    \hline
  & \multicolumn{3}{c|}{Vicuna-7b-v1.5} & \multicolumn{3}{c|}{GPT-3.5-turbo} & \multicolumn{3}{c|}{GPT-4-1106-preview} \\
    \hline
 & P & Recall & F1 & P & Recall & F1 & P & Recall & F1 \\
 \hline
 
 
 Basic &  0.801 & 0.475 & 0.571 & 0.898 & 0.620 & 0.716 & 0.996 & 0.729 & 0.833
 
 \\
 % Explain & 0.769 & 0.621 & 0.648 & 0.598 & 0.856 & 0.672 \\
 Extended &  \textbf{0.945} & \textbf{0.627} & \textbf{0.714} & \textbf{0.978} & \textbf{0.646} & \textbf{0.764} & \textbf{0.996} & \textbf{0.735} & \textbf{0.841}
\\
 \hline
\end{tabular}
\end{adjustbox}

==> figures/prompt_evaluation_full.tex <==
\caption{\textsc{Storyline labelling performance for \basicprompt and \extendedprompt}}
 \extendedprompt &   \textbf{0.687} & \textbf{0.738} & \textbf{0.715} 
\begin{adjustbox}{width=1\linewidth}

\begin{tabular}{ |c|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|} 
    \hline
  & \multicolumn{9}{c|}{Vicuna-7b-v1.5} & \multicolumn{9}{c|}{GPT-3.5-turbo} & \multicolumn{9}{c|}{GPT-4-1106-preview} \\
    \hline
    dataset & \multicolumn{9}{c|}{crisis} & \multicolumn{9}{c|}{TL17} & \multicolumn{9}{c|}{Finance News} \\
    \hline
 & P & Recall & F1 & P & Recall & F1 & P & Recall & F1  & P & Recall & F1 & P & Recall & F1 & P & Recall & F1
 & P & Recall & F1 & P & Recall & F1 & P & Recall & F1
  \\
 \hline
 
 
 Basic &  0.661 & 0.452 & 0.516 & 0.886 & 0.491 & 0.594 & 0.818 & 0.477 & 0.583 & 0.873 & 0.672 & 0.738 & 0.781 & 0.602 & 0.671 & 0.963 & 0.607 & 0.728 & 1.000 & 0.764 & 0.865 & 1.000 & 0.739 & 0.841 & 0.993 & 0.711 & 0.817

 
 \\
 % Explain & 0.769 & 0.621 & 0.648 & 0.598 & 0.856 & 0.672 \\
 Extended &   0.930 & 0.593 & 0.687 & 0.945 & 0.673 & 0.738 & 0.951 & 0.620 & 0.715 & 0.987 & 0.711 & 0.819 & 0.962 & 0.611 & 0.730 & 0.982 & 0.637 & 0.758 & 1.000 & 0.764 & 0.865 & 1.000 & 0.748 & 0.852 & 0.993 & 0.716 & 0.827

\\
 \hline
\end{tabular}
\end{adjustbox}

==> figures/prompt_evaluation_one_column.tex <==
% \caption{\textsc{Storyline labelling performance for \basicprompt and \extendedprompt}}
%  \extendedprompt &   \textbf{0.687} & \textbf{0.738} & \textbf{0.715} 


\begin{tabular}{ |c|ccc|} 
  %   \hline
  % & \multicolumn{3}{c|}{Vicuna-7b-v1.5} & \multicolumn{3}{c|}{GPT-3.5-turbo} & \multicolumn{3}{c|}{GPT-4-1106-preview} \\
    \hline
 & P & Recall & F1  \\
 \hline
 & \multicolumn{3}{c|}{Vicuna-7b-v1.5} \\
 
 Basic &  0.801 & 0.475 & 0.571
 
 \\
 % Explain & 0.769 & 0.621 & 0.648 & 0.598 & 0.856 & 0.672 \\
 Extended &  \textbf{0.945} & \textbf{0.627} & \textbf{0.714} 
\\
 \hline


 & \multicolumn{3}{c|}{GPT-3.5-turbo} \\
 
 Basic & 0.898 & 0.620 & 0.716 
 
 \\
 % Explain & 0.769 & 0.621 & 0.648 & 0.598 & 0.856 & 0.672 \\
 Extended & \textbf{0.978} & \textbf{0.646} & \textbf{0.764} 
\\
 \hline


& \multicolumn{3}{c|}{GPT-4-1106-preview} \\
 
 Basic &  0.996 & 0.729 & 0.833 
 
 \\
 % Explain & 0.769 & 0.621 & 0.648 & 0.598 & 0.856 & 0.672 \\
 Extended & \textbf{0.996} & \textbf{0.735} & \textbf{0.841} 
\\
 \hline
\end{tabular}

